Do Investors Hedge Against Green Swans? Option-Implied Risk Aversion to Wildfires

Measuring beliefs about natural disasters is challenging. Deep out-of-the-money options allow investors to hedge at a range of strikes and time horizons, thus the 3-dimensional surface of firm-level option prices provides information on (i) skewed and fat-tailed beliefs about the impact of natural disaster risk across space and time dimensions at daily frequency; and (ii) information on the covariance of wildfire-exposed stocks with investors' marginal utility of wealth. Each publicly-traded company's daily surface of option prices is matched with its network of establishments and wildfire perimeters over two decades. First, wildfires affect investors' risk neutral probabilities at short and long maturities; investors price asymmetric downward tail risk and a probability of upward jumps. The volatility smile is more pronounced. Second, comparing risk-neutral and physical distributions reveals the option-implied risk aversion with respect to wildfire-exposed stock prices. Investors' marginal utility of wealth is correlated with wildfire shocks. Option-implied risk aversion identifies the wildfire-exposed share of portfolios. For risk aversions consistent with Barro (2012), equity options suggest (i) investors hold larger shares of wildfire-exposed stocks than the market portfolio; or (ii) investors may have more pessimistic beliefs about wildfires' impacts than what observed returns suggest, such as pricing low-probability unrealized downward tail risk. We calibrate options with models featuring both upward and downward risk. Results are consistent a significant pricing of downward jumps.

==> tables/ambiguity.tex <==
\begin{tabular}{lcccc}
    \toprule
                             & \multicolumn{1}{c}{$\mathbf{1}(K/S<0.2)_{i,t}$} & \multicolumn{1}{c}{$\mathbf{1}(K/S<0.5)_{i,t}$} & 
                             \multicolumn{1}{c}{$\mathbf{1}(K/S>1.5)_{i,t}$} & \multicolumn{1}{c}{$\mathbf{1}(K/S>1.8)_{i,t}$} \\
    \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5}
                             &                                                 (1) &
      (2) &                                                 (3) &                                                 (4) \\
    \midrule
    maturity\_100            &                                            0.001*** &                                            0.004*** &                                            0.003*** &                                            0.001*** \\
                             &                                             (0.000) &                                             (0.000) &                                             (0.000) &                                             (0.000) \\
    treated                  &                                               0.001 &                                             0.009** &                                               0.001 &                                               0.004 \\
                             &                                             (0.001) &                                             (0.003) &                                             (0.005) &                                             (0.003) \\
    treated \& maturity\_100 &                                              -0.000 &                                            -0.001** &                                              -0.000 &                                            -0.001** \\
                             &                                             (0.000) &                                             (0.000) &                                             (0.000) &                                             (0.000) \\
    \midrule
    date                     &                                                 Yes &
      Yes &                                                 Yes &                                                 Yes \\
    ticker                   &                                                 Yes &
      Yes &                                                 Yes &                                                 Yes \\
    \midrule
    Estimator                &                                                 OLS &
      OLS &                                                 OLS &                                                 OLS \\
    \midrule
    $N$                      &                                          16,842,463 &                                          16,842,463 &                                          16,839,339 &                                          16,839,339 \\
    $R^2$                    &                                               0.035 &
    0.054 &                                               0.116 &                                               0.091 \\
    \bottomrule
    \end{tabular}
    

==> tables/impact_RND_by_moneyness.tex <==
\begin{tabular}{lcc}
\tabularnewline\hline\hline

Dependent Variable:&\multicolumn{2}{c}{logit\_w}\\

Model:&(1)&(2)\\

\hline
\emph{Variables}&  & \\

moneyness\_cut(0.445,0.4977]&-0.1596&0.4164$^{***}$\\
  &(0.1735)&(0.1156)\\
moneyness\_cut(0.4977,0.5296]&0.1347&0.7941$^{***}$\\
  &(0.2014)&(0.1303)\\
moneyness\_cut(0.5296,0.5539]&0.1550&1.213$^{***}$\\
  &(0.2068)&(0.1396)\\
moneyness\_cut(0.5539,0.5745]&0.5139$^{**}$&1.559$^{***}$\\
  &(0.2140)&(0.1443)\\
moneyness\_cut(0.5745,0.593]&0.5711$^{***}$&1.741$^{***}$\\
  &(0.2102)&(0.1484)\\
moneyness\_cut(0.593,0.61]&0.8438$^{***}$&1.893$^{***}$\\
  &(0.2177)&(0.1480)\\
moneyness\_cut(0.61,0.6257]&1.233$^{***}$&2.139$^{***}$\\
  &(0.2210)&(0.1514)\\
moneyness\_cut(0.6257,0.6406]&0.9742$^{***}$&2.176$^{***}$\\
  &(0.2159)&(0.1486)\\
moneyness\_cut(0.6406,0.6547]&1.399$^{***}$&2.344$^{***}$\\
  &(0.2217)&(0.1510)\\
moneyness\_cut(0.6547,0.6681]&1.336$^{***}$&2.569$^{***}$\\
  &(0.2190)&(0.1517)\\
moneyness\_cut(0.6681,0.681]&1.27$^{***}$&2.611$^{***}$\\
  &(0.2158)&(0.1545)\\
moneyness\_cut(0.681,0.6933]&1.383$^{***}$&2.428$^{***}$\\
  &(0.2115)&(0.1472)\\
moneyness\_cut(0.6933,0.7051]&1.468$^{***}$&2.71$^{***}$\\
  &(0.2156)&(0.1517)\\
moneyness\_cut(0.7051,0.7165]&1.532$^{***}$&2.884$^{***}$\\
  &(0.2202)&(0.1529)\\
moneyness\_cut(0.7165,0.7275]&1.663$^{***}$&2.966$^{***}$\\
  &(0.2174)&(0.1474)\\
moneyness\_cut(0.7275,0.7382]&1.661$^{***}$&3.129$^{***}$\\
  &(0.2144)&(0.1481)\\
moneyness\_cut(0.7382,0.7485]&1.589$^{***}$&3.092$^{***}$\\
  &(0.2143)&(0.1452)\\
moneyness\_cut(0.7485,0.7586]&1.475$^{***}$&3.148$^{***}$\\
  &(0.2060)&(0.1443)\\
moneyness\_cut(0.7586,0.7683]&1.616$^{***}$&3.194$^{***}$\\
  &(0.2157)&(0.1474)\\
moneyness\_cut(0.7683,0.7778]&1.77$^{***}$&3.253$^{***}$\\
  &(0.2129)&(0.1414)\\
moneyness\_cut(0.7778,0.7871]&1.669$^{***}$&3.251$^{***}$\\
  &(0.2116)&(0.1441)\\
moneyness\_cut(0.7871,0.7962]&1.807$^{***}$&3.236$^{***}$\\
  &(0.2159)&(0.1425)\\
moneyness\_cut(0.7962,0.805]&1.685$^{***}$&3.135$^{***}$\\
  &(0.2136)&(0.1399)\\
moneyness\_cut(0.805,0.8136]&1.773$^{***}$&3.32$^{***}$\\
  &(0.2077)&(0.1364)\\
moneyness\_cut(0.8136,0.822]&1.87$^{***}$&3.634$^{***}$\\
  &(0.2116)&(0.1404)\\
moneyness\_cut(0.822,0.8303]&1.827$^{***}$&3.634$^{***}$\\
  &(0.2201)&(0.1495)\\
moneyness\_cut(0.8303,0.8384]&1.862$^{***}$&3.533$^{***}$\\
  &(0.2143)&(0.1488)\\
moneyness\_cut(0.8384,0.8464]&1.836$^{***}$&3.491$^{***}$\\
  &(0.2142)&(0.1507)\\
moneyness\_cut(0.8464,0.8543]&1.853$^{***}$&3.603$^{***}$\\
  &(0.2074)&(0.1475)\\
moneyness\_cut(0.8543,0.862]&1.975$^{***}$&3.582$^{***}$\\
  &(0.2096)&(0.1432)\\
moneyness\_cut(0.862,0.8696]&1.897$^{***}$&3.525$^{***}$\\
  &(0.2100)&(0.1488)\\
moneyness\_cut(0.8696,0.8771]&1.875$^{***}$&3.517$^{***}$\\
  &(0.2122)&(0.1408)\\
moneyness\_cut(0.8771,0.8845]&1.97$^{***}$&3.571$^{***}$\\
  &(0.2108)&(0.1406)\\
moneyness\_cut(0.8845,0.8919]&2.122$^{***}$&3.758$^{***}$\\
  &(0.2078)&(0.1383)\\
moneyness\_cut(0.8919,0.8991]&2.038$^{***}$&3.772$^{***}$\\
  &(0.2076)&(0.1441)\\
moneyness\_cut(0.8991,0.9063]&2.094$^{***}$&3.808$^{***}$\\
  &(0.2101)&(0.1463)\\
moneyness\_cut(0.9063,0.9135]&2.112$^{***}$&3.846$^{***}$\\
  &(0.2131)&(0.1437)\\
moneyness\_cut(0.9135,0.9205]&2.075$^{***}$&3.853$^{***}$\\
  &(0.2131)&(0.1455)\\
moneyness\_cut(0.9205,0.9276]&2.106$^{***}$&3.907$^{***}$\\
  &(0.2138)&(0.1490)\\
moneyness\_cut(0.9276,0.9345]&2.309$^{***}$&3.955$^{***}$\\
  &(0.2074)&(0.1503)\\
moneyness\_cut(0.9345,0.9414]&2.364$^{***}$&3.959$^{***}$\\
  &(0.2105)&(0.1481)\\
moneyness\_cut(0.9414,0.9483]&2.465$^{***}$&3.994$^{***}$\\
  &(0.2075)&(0.1526)\\
moneyness\_cut(0.9483,0.9552]&2.472$^{***}$&4.019$^{***}$\\
  &(0.2084)&(0.1512)\\
moneyness\_cut(0.9552,0.962]&2.462$^{***}$&4.042$^{***}$\\
  &(0.2070)&(0.1508)\\
moneyness\_cut(0.962,0.9689]&2.473$^{***}$&4.119$^{***}$\\
  &(0.2098)&(0.1503)\\
moneyness\_cut(0.9689,0.9756]&2.568$^{***}$&4.085$^{***}$\\
  &(0.2050)&(0.1434)\\
moneyness\_cut(0.9756,0.9824]&2.501$^{***}$&4.039$^{***}$\\
  &(0.2106)&(0.1397)\\
moneyness\_cut(0.9824,0.9892]&2.531$^{***}$&4.19$^{***}$\\
  &(0.2117)&(0.1449)\\
moneyness\_cut(0.9892,0.9959]&2.515$^{***}$&4.156$^{***}$\\
  &(0.2117)&(0.1438)\\
moneyness\_cut(0.9959,1.003]&2.533$^{***}$&4.281$^{***}$\\
  &(0.2071)&(0.1467)\\
moneyness\_cut(1.003,1.009]&2.612$^{***}$&4.204$^{***}$\\
  &(0.2088)&(0.1456)\\
moneyness\_cut(1.009,1.016]&2.58$^{***}$&4.251$^{***}$\\
  &(0.2097)&(0.1529)\\
moneyness\_cut(1.016,1.023]&2.718$^{***}$&4.326$^{***}$\\
  &(0.2070)&(0.1499)\\
moneyness\_cut(1.023,1.03]&2.619$^{***}$&4.27$^{***}$\\
  &(0.2026)&(0.1549)\\
moneyness\_cut(1.03,1.037]&2.697$^{***}$&4.419$^{***}$\\
  &(0.2121)&(0.1528)\\
moneyness\_cut(1.037,1.043]&2.751$^{***}$&4.419$^{***}$\\
  &(0.2025)&(0.1514)\\
moneyness\_cut(1.043,1.05]&2.856$^{***}$&4.461$^{***}$\\
  &(0.2056)&(0.1515)\\
moneyness\_cut(1.05,1.057]&2.759$^{***}$&4.505$^{***}$\\
  &(0.2084)&(0.1558)\\
moneyness\_cut(1.057,1.064]&2.852$^{***}$&4.413$^{***}$\\
  &(0.2023)&(0.1584)\\
moneyness\_cut(1.064,1.071]&2.985$^{***}$&4.458$^{***}$\\
  &(0.2042)&(0.1539)\\
moneyness\_cut(1.071,1.078]&2.97$^{***}$&4.608$^{***}$\\
  &(0.2043)&(0.1572)\\
moneyness\_cut(1.078,1.086]&2.897$^{***}$&4.647$^{***}$\\
  &(0.2088)&(0.1600)\\
moneyness\_cut(1.086,1.093]&2.827$^{***}$&4.687$^{***}$\\
  &(0.2026)&(0.1599)\\
moneyness\_cut(1.093,1.1]&2.807$^{***}$&4.634$^{***}$\\
  &(0.2046)&(0.1601)\\
moneyness\_cut(1.1,1.108]&2.874$^{***}$&4.69$^{***}$\\
  &(0.2095)&(0.1652)\\
moneyness\_cut(1.108,1.115]&2.885$^{***}$&4.769$^{***}$\\
  &(0.2112)&(0.1607)\\
moneyness\_cut(1.115,1.123]&2.866$^{***}$&4.804$^{***}$\\
  &(0.2090)&(0.1632)\\
moneyness\_cut(1.123,1.131]&2.726$^{***}$&4.905$^{***}$\\
  &(0.2132)&(0.1665)\\
moneyness\_cut(1.131,1.139]&2.845$^{***}$&4.895$^{***}$\\
  &(0.2106)&(0.1792)\\
moneyness\_cut(1.139,1.148]&2.833$^{***}$&4.821$^{***}$\\
  &(0.2091)&(0.1676)\\
moneyness\_cut(1.148,1.156]&2.858$^{***}$&4.909$^{***}$\\
  &(0.2157)&(0.1673)\\
moneyness\_cut(1.156,1.165]&2.979$^{***}$&5.009$^{***}$\\
  &(0.2124)&(0.1739)\\
moneyness\_cut(1.165,1.174]&3.004$^{***}$&5.323$^{***}$\\
  &(0.2069)&(0.1730)\\
moneyness\_cut(1.174,1.184]&2.862$^{***}$&5.49$^{***}$\\
  &(0.2018)&(0.1812)\\
moneyness\_cut(1.184,1.193]&2.982$^{***}$&5.378$^{***}$\\
  &(0.2075)&(0.1845)\\
moneyness\_cut(1.193,1.203]&3.061$^{***}$&5.269$^{***}$\\
  &(0.2153)&(0.1813)\\
moneyness\_cut(1.203,1.213]&3.011$^{***}$&5.267$^{***}$\\
  &(0.2133)&(0.1828)\\
moneyness\_cut(1.213,1.224]&2.962$^{***}$&5.522$^{***}$\\
  &(0.2079)&(0.1950)\\
moneyness\_cut(1.224,1.235]&3.048$^{***}$&5.72$^{***}$\\
  &(0.2175)&(0.1955)\\
moneyness\_cut(1.235,1.246]&3.216$^{***}$&5.715$^{***}$\\
  &(0.2209)&(0.2002)\\
moneyness\_cut(1.246,1.258]&3.436$^{***}$&5.757$^{***}$\\
  &(0.2266)&(0.1902)\\
moneyness\_cut(1.258,1.27]&3.447$^{***}$&5.986$^{***}$\\
  &(0.2329)&(0.1992)\\
moneyness\_cut(1.27,1.282]&3.58$^{***}$&6.027$^{***}$\\
  &(0.2356)&(0.2090)\\
moneyness\_cut(1.282,1.295]&3.692$^{***}$&6.322$^{***}$\\
  &(0.2297)&(0.2062)\\
moneyness\_cut(1.295,1.309]&3.456$^{***}$&6.655$^{***}$\\
  &(0.2246)&(0.2243)\\
moneyness\_cut(1.309,1.324]&3.635$^{***}$&6.691$^{***}$\\
  &(0.2388)&(0.2263)\\
moneyness\_cut(1.324,1.339]&3.591$^{***}$&6.848$^{***}$\\
  &(0.2324)&(0.2345)\\
moneyness\_cut(1.339,1.355]&3.675$^{***}$&6.882$^{***}$\\
  &(0.2423)&(0.2381)\\
moneyness\_cut(1.355,1.373]&4.006$^{***}$&6.814$^{***}$\\
  &(0.2499)&(0.2616)\\
moneyness\_cut(1.373,1.392]&3.99$^{***}$&6.756$^{***}$\\
  &(0.2466)&(0.2614)\\
moneyness\_cut(1.392,1.414]&3.94$^{***}$&6.789$^{***}$\\
  &(0.2541)&(0.2651)\\
moneyness\_cut(1.414,1.438]&4.013$^{***}$&6.804$^{***}$\\
  &(0.2622)&(0.2665)\\
moneyness\_cut(1.438,1.467]&4.124$^{***}$&6.888$^{***}$\\
  &(0.2593)&(0.2801)\\
moneyness\_cut(1.467,1.502]&4.082$^{***}$&6.815$^{***}$\\
  &(0.2722)&(0.3012)\\
moneyness\_cut(1.502,1.547]&3.763$^{***}$&6.584$^{***}$\\
  &(0.2791)&(0.3050)\\
moneyness\_cut(1.547,1.608]&3.773$^{***}$&6.732$^{***}$\\
  &(0.2887)&(0.3312)\\
moneyness\_cut(1.608,1.696]&3.724$^{***}$&6.683$^{***}$\\
  &(0.3061)&(0.3515)\\
moneyness\_cut(1.696,1.844]&3.578$^{***}$&6.152$^{***}$\\
  &(0.3360)&(0.3842)\\
moneyness\_cut(1.844,2.499]&3.869$^{***}$&6.114$^{***}$\\
  &(0.4024)&(0.4819)\\
treated $\times $ moneyness\_cut(0.2001,0.445]&-0.7274$^{*}$&-0.3588\\
  &(0.4067)&(0.4180)\\
treated $\times $ moneyness\_cut(0.445,0.4977]&-0.3961&-0.2187\\
  &(0.3110)&(0.3027)\\
treated $\times $ moneyness\_cut(0.4977,0.5296]&-0.2893&-0.0674\\
  &(0.2981)&(0.2794)\\
treated $\times $ moneyness\_cut(0.5296,0.5539]&-0.0106&-0.0691\\
  &(0.2519)&(0.2583)\\
treated $\times $ moneyness\_cut(0.5539,0.5745]&-0.1167&-0.2905\\
  &(0.2696)&(0.2503)\\
treated $\times $ moneyness\_cut(0.5745,0.593]&0.2905&0.0738\\
  &(0.2453)&(0.2431)\\
treated $\times $ moneyness\_cut(0.593,0.61]&-0.1088&-0.1327\\
  &(0.2275)&(0.2364)\\
treated $\times $ moneyness\_cut(0.61,0.6257]&-0.5485$^{**}$&-0.3941$^{*}$\\
  &(0.2235)&(0.2131)\\
treated $\times $ moneyness\_cut(0.6257,0.6406]&-0.0306&-0.2164\\
  &(0.2138)&(0.2091)\\
treated $\times $ moneyness\_cut(0.6406,0.6547]&-0.0696&0.0016\\
  &(0.2140)&(0.2209)\\
treated $\times $ moneyness\_cut(0.6547,0.6681]&0.0552&-0.1850\\
  &(0.2129)&(0.1848)\\
treated $\times $ moneyness\_cut(0.6681,0.681]&0.1291&-0.0588\\
  &(0.2197)&(0.2028)\\
treated $\times $ moneyness\_cut(0.681,0.6933]&0.0507&0.2139\\
  &(0.1962)&(0.1937)\\
treated $\times $ moneyness\_cut(0.6933,0.7051]&-0.0499&-0.1734\\
  &(0.1922)&(0.1938)\\
treated $\times $ moneyness\_cut(0.7051,0.7165]&0.0807&-0.2192\\
  &(0.1936)&(0.2083)\\
treated $\times $ moneyness\_cut(0.7165,0.7275]&-0.1811&-0.2021\\
  &(0.1890)&(0.1835)\\
treated $\times $ moneyness\_cut(0.7275,0.7382]&0.1446&-0.1566\\
  &(0.1934)&(0.1837)\\
treated $\times $ moneyness\_cut(0.7382,0.7485]&0.2577&-0.0775\\
  &(0.1985)&(0.1872)\\
treated $\times $ moneyness\_cut(0.7485,0.7586]&0.2292&-0.0597\\
  &(0.1924)&(0.1862)\\
treated $\times $ moneyness\_cut(0.7586,0.7683]&-0.0110&-0.2217\\
  &(0.1828)&(0.1705)\\
treated $\times $ moneyness\_cut(0.7683,0.7778]&-0.1408&-0.1841\\
  &(0.1808)&(0.1755)\\
treated $\times $ moneyness\_cut(0.7778,0.7871]&0.1682&-0.0811\\
  &(0.1588)&(0.1788)\\
treated $\times $ moneyness\_cut(0.7871,0.7962]&0.0781&-0.0220\\
  &(0.1729)&(0.1864)\\
treated $\times $ moneyness\_cut(0.7962,0.805]&-0.0693&0.0001\\
  &(0.1683)&(0.1786)\\
treated $\times $ moneyness\_cut(0.805,0.8136]&-0.0300&-0.0316\\
  &(0.1795)&(0.1696)\\
treated $\times $ moneyness\_cut(0.8136,0.822]&0.0057&-0.1185\\
  &(0.1745)&(0.1717)\\
treated $\times $ moneyness\_cut(0.822,0.8303]&0.0297&-0.0837\\
  &(0.1706)&(0.1563)\\
treated $\times $ moneyness\_cut(0.8303,0.8384]&-0.0789&-0.0255\\
  &(0.1762)&(0.1600)\\
treated $\times $ moneyness\_cut(0.8384,0.8464]&0.0741&-0.0141\\
  &(0.1693)&(0.1679)\\
treated $\times $ moneyness\_cut(0.8464,0.8543]&0.0152&-0.2279\\
  &(0.1633)&(0.1739)\\
treated $\times $ moneyness\_cut(0.8543,0.862]&-0.1000&-0.0890\\
  &(0.1735)&(0.1808)\\
treated $\times $ moneyness\_cut(0.862,0.8696]&-0.1134&-0.0550\\
  &(0.1736)&(0.1878)\\
treated $\times $ moneyness\_cut(0.8696,0.8771]&0.2233&0.1065\\
  &(0.1715)&(0.1774)\\
treated $\times $ moneyness\_cut(0.8771,0.8845]&0.4264$^{**}$&0.3954$^{**}$\\
  &(0.1689)&(0.1740)\\
treated $\times $ moneyness\_cut(0.8845,0.8919]&0.2036&0.1947\\
  &(0.1585)&(0.1705)\\
treated $\times $ moneyness\_cut(0.8919,0.8991]&0.1407&0.0469\\
  &(0.1616)&(0.1588)\\
treated $\times $ moneyness\_cut(0.8991,0.9063]&0.0856&0.0768\\
  &(0.1740)&(0.1660)\\
treated $\times $ moneyness\_cut(0.9063,0.9135]&0.2061&0.0898\\
  &(0.1585)&(0.1565)\\
treated $\times $ moneyness\_cut(0.9135,0.9205]&0.3283$^{**}$&0.0776\\
  &(0.1604)&(0.1694)\\
treated $\times $ moneyness\_cut(0.9205,0.9276]&0.1826&0.0380\\
  &(0.1590)&(0.1532)\\
treated $\times $ moneyness\_cut(0.9276,0.9345]&-0.1211&-0.0908\\
  &(0.1601)&(0.1631)\\
treated $\times $ moneyness\_cut(0.9345,0.9414]&-0.1472&-0.0965\\
  &(0.1540)&(0.1643)\\
treated $\times $ moneyness\_cut(0.9414,0.9483]&-0.1886&-0.0516\\
  &(0.1589)&(0.1650)\\
treated $\times $ moneyness\_cut(0.9483,0.9552]&0.0402&0.1247\\
  &(0.1536)&(0.1743)\\
treated $\times $ moneyness\_cut(0.9552,0.962]&0.1026&0.2033\\
  &(0.1611)&(0.1700)\\
treated $\times $ moneyness\_cut(0.962,0.9689]&0.0128&-0.0185\\
  &(0.1582)&(0.1620)\\
treated $\times $ moneyness\_cut(0.9689,0.9756]&-0.1873&0.0381\\
  &(0.1411)&(0.1560)\\
treated $\times $ moneyness\_cut(0.9756,0.9824]&-0.0052&0.1224\\
  &(0.1573)&(0.1497)\\
treated $\times $ moneyness\_cut(0.9824,0.9892]&0.1855&0.1707\\
  &(0.1527)&(0.1608)\\
treated $\times $ moneyness\_cut(0.9892,0.9959]&0.2883$^{*}$&0.2472\\
  &(0.1575)&(0.1579)\\
treated $\times $ moneyness\_cut(0.9959,1.003]&0.4174$^{**}$&0.2551\\
  &(0.1655)&(0.1677)\\
treated $\times $ moneyness\_cut(1.003,1.009]&0.2280&0.2780$^{*}$\\
  &(0.1543)&(0.1645)\\
treated $\times $ moneyness\_cut(1.009,1.016]&0.1709&0.3291$^{**}$\\
  &(0.1479)&(0.1648)\\
treated $\times $ moneyness\_cut(1.016,1.023]&-0.0760&0.0971\\
  &(0.1642)&(0.1680)\\
treated $\times $ moneyness\_cut(1.023,1.03]&-0.0834&0.1415\\
  &(0.1631)&(0.1823)\\
treated $\times $ moneyness\_cut(1.03,1.037]&-0.0784&-0.0289\\
  &(0.1613)&(0.1771)\\
treated $\times $ moneyness\_cut(1.037,1.043]&0.0384&0.1448\\
  &(0.1727)&(0.1732)\\
treated $\times $ moneyness\_cut(1.043,1.05]&0.0069&0.0977\\
  &(0.1625)&(0.1620)\\
treated $\times $ moneyness\_cut(1.05,1.057]&0.0241&0.0246\\
  &(0.1709)&(0.1632)\\
treated $\times $ moneyness\_cut(1.057,1.064]&-0.1129&0.0966\\
  &(0.1551)&(0.1672)\\
treated $\times $ moneyness\_cut(1.064,1.071]&-0.1357&0.1203\\
  &(0.1520)&(0.1659)\\
treated $\times $ moneyness\_cut(1.071,1.078]&-0.0713&0.1131\\
  &(0.1539)&(0.1799)\\
treated $\times $ moneyness\_cut(1.078,1.086]&0.0882&0.2177\\
  &(0.1597)&(0.1817)\\
treated $\times $ moneyness\_cut(1.086,1.093]&0.0271&0.0402\\
  &(0.1523)&(0.1775)\\
treated $\times $ moneyness\_cut(1.093,1.1]&0.0091&0.0776\\
  &(0.1596)&(0.1844)\\
treated $\times $ moneyness\_cut(1.1,1.108]&-0.0285&0.1294\\
  &(0.1694)&(0.1807)\\
treated $\times $ moneyness\_cut(1.108,1.115]&0.0100&0.1960\\
  &(0.1670)&(0.1849)\\
treated $\times $ moneyness\_cut(1.115,1.123]&0.0211&0.2059\\
  &(0.1729)&(0.2044)\\
treated $\times $ moneyness\_cut(1.123,1.131]&0.2186&0.1848\\
  &(0.1565)&(0.1939)\\
treated $\times $ moneyness\_cut(1.131,1.139]&0.1352&0.2490\\
  &(0.1500)&(0.1858)\\
treated $\times $ moneyness\_cut(1.139,1.148]&0.1538&0.4003$^{**}$\\
  &(0.1607)&(0.2016)\\
treated $\times $ moneyness\_cut(1.148,1.156]&0.1719&0.5262$^{***}$\\
  &(0.1629)&(0.1962)\\
treated $\times $ moneyness\_cut(1.156,1.165]&0.1481&0.4781$^{**}$\\
  &(0.1724)&(0.2128)\\
treated $\times $ moneyness\_cut(1.165,1.174]&-0.0621&-0.0099\\
  &(0.1810)&(0.2268)\\
treated $\times $ moneyness\_cut(1.174,1.184]&0.0777&-0.2976\\
  &(0.1966)&(0.2448)\\
treated $\times $ moneyness\_cut(1.184,1.193]&-0.1141&-0.1623\\
  &(0.1905)&(0.2344)\\
treated $\times $ moneyness\_cut(1.193,1.203]&-0.0899&0.1167\\
  &(0.1804)&(0.2475)\\
treated $\times $ moneyness\_cut(1.203,1.213]&0.1786&0.3480\\
  &(0.1953)&(0.2377)\\
treated $\times $ moneyness\_cut(1.213,1.224]&0.4486$^{**}$&0.4560$^{*}$\\
  &(0.1912)&(0.2400)\\
treated $\times $ moneyness\_cut(1.224,1.235]&0.3195&0.2825\\
  &(0.1983)&(0.2377)\\
treated $\times $ moneyness\_cut(1.235,1.246]&-0.0189&0.2502\\
  &(0.2037)&(0.2422)\\
treated $\times $ moneyness\_cut(1.246,1.258]&-0.5141$^{**}$&0.0966\\
  &(0.2109)&(0.2463)\\
treated $\times $ moneyness\_cut(1.258,1.27]&-0.2835&-0.1972\\
  &(0.2235)&(0.2527)\\
treated $\times $ moneyness\_cut(1.27,1.282]&-0.4146$^{*}$&-0.0120\\
  &(0.2295)&(0.2657)\\
treated $\times $ moneyness\_cut(1.282,1.295]&-0.3734&-0.1961\\
  &(0.2516)&(0.2833)\\
treated $\times $ moneyness\_cut(1.295,1.309]&0.2720&-0.0930\\
  &(0.2554)&(0.2937)\\
treated $\times $ moneyness\_cut(1.309,1.324]&0.0811&-0.4855$^{*}$\\
  &(0.2389)&(0.2668)\\
treated $\times $ moneyness\_cut(1.324,1.339]&-0.2047&-0.6541$^{**}$\\
  &(0.2434)&(0.2984)\\
treated $\times $ moneyness\_cut(1.339,1.355]&-0.3210&-0.6469$^{**}$\\
  &(0.2666)&(0.3095)\\
treated $\times $ moneyness\_cut(1.355,1.373]&-0.3929&-0.3799\\
  &(0.2725)&(0.3353)\\
treated $\times $ moneyness\_cut(1.373,1.392]&-0.3242&-0.0820\\
  &(0.3119)&(0.3395)\\
treated $\times $ moneyness\_cut(1.392,1.414]&-0.2437&-0.0595\\
  &(0.3229)&(0.3741)\\
treated $\times $ moneyness\_cut(1.414,1.438]&-0.5032$^{*}$&-0.0768\\
  &(0.2960)&(0.3525)\\
treated $\times $ moneyness\_cut(1.438,1.467]&-0.5173$^{*}$&0.1127\\
  &(0.2914)&(0.3987)\\
treated $\times $ moneyness\_cut(1.467,1.502]&-0.3366&-0.3160\\
  &(0.3196)&(0.3974)\\
treated $\times $ moneyness\_cut(1.502,1.547]&0.1922&0.5218\\
  &(0.3878)&(0.4265)\\
treated $\times $ moneyness\_cut(1.547,1.608]&-0.0508&0.0644\\
  &(0.3767)&(0.4282)\\
treated $\times $ moneyness\_cut(1.608,1.696]&0.0029&0.1997\\
  &(0.4354)&(0.5374)\\
treated $\times $ moneyness\_cut(1.696,1.844]&0.0614&0.3331\\
  &(0.5493)&(0.6461)\\
treated $\times $ moneyness\_cut(1.844,2.499]&-0.5094&-0.3931\\
  &(0.8719)&(1.053)\\

\hline
\emph{Fixed-effects}&  & \\

ticker&Yes&Yes\\
date&Yes&Yes\\

\hline
\emph{Fit statistics}&  & \\
Observations& 701,276&689,450\\
R$^2$ & 0.19742&0.24006\\
Within R$^2$ & 0.03424&0.09198\\

\hline\hline
\multicolumn{3}{l}{\emph{One-way (ticker) standard-errors in parentheses}}\\
\multicolumn{3}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\

\end{tabular}



==> tables/table_linear_results.tex <==
\begin{tabular}{lccc}
\tabularnewline\hline\hline

Dependent Variable:&\multicolumn{3}{c}{rnd}\\

Model:&(1)&(2)&(3)\\

\hline
\emph{Variables}&  & & \\

treated&-0.0057$^{*}$&  &  \\
  &(0.0031)&  &  \\
moneyness\_more\_1&-0.0003&-0.0018&0.0015\\
  &(0.0012)&(0.0014)&(0.0014)\\
maturity&$-2.339\times 10^{-5}$$^{***}$&$-2.892\times 10^{-5}$$^{***}$&$-1.53\times 10^{-5}$$^{***}$\\
  &($5.679\times 10^{-6}$)&($6.307\times 10^{-6}$)&($4.659\times 10^{-6}$)\\
moneyness\_less\_1&0.0043$^{***}$&0.0029&0.0065$^{***}$\\
  &(0.0016)&(0.0018)&(0.0018)\\
treated $\times $ moneyness\_more\_1&0.0050$^{*}$&  &  \\
  &(0.0027)&  &  \\
treated $\times $ maturity&$1.674\times 10^{-5}$$^{**}$&  &  \\
  &($6.943\times 10^{-6}$)&  &  \\
moneyness\_more\_1 $\times $ maturity&$5.944\times 10^{-6}$&$1.02\times 10^{-5}$$^{*}$&$-1.413\times 10^{-6}$\\
  &($4.653\times 10^{-6}$)&($5.58\times 10^{-6}$)&($3.539\times 10^{-6}$)\\
treated $\times $ moneyness\_less\_1&0.0059$^{*}$&  &  \\
  &(0.0035)&  &  \\
maturity $\times $ moneyness\_less\_1&$-3.35\times 10^{-6}$&$2.238\times 10^{-6}$&$-1.379\times 10^{-5}$$^{***}$\\
  &($6.469\times 10^{-6}$)&($7.646\times 10^{-6}$)&($4.911\times 10^{-6}$)\\
treated $\times $ moneyness\_more\_1 $\times $ maturity&$-1.604\times 10^{-5}$$^{**}$&  &  \\
  &($6.348\times 10^{-6}$)&  &  \\
treated $\times $ maturity $\times $ moneyness\_less\_1&$-2.179\times 10^{-5}$$^{***}$&  &  \\
  &($8.313\times 10^{-6}$)&  &  \\
after\_treated\_1st&  &-0.0074$^{**}$&  \\
  &  &(0.0029)&  \\
after\_treated\_1st $\times $ moneyness\_more\_1&  &0.0066$^{***}$&  \\
  &  &(0.0024)&  \\
after\_treated\_1st $\times $ maturity&  &$2.274\times 10^{-5}$$^{***}$&  \\
  &  &($8.218\times 10^{-6}$)&  \\
after\_treated\_1st $\times $ moneyness\_less\_1&  &0.0073$^{**}$&  \\
  &  &(0.0031)&  \\
after\_treated\_1st $\times $ moneyness\_more\_1 $\times $ maturity&  &$-2.024\times 10^{-5}$$^{***}$&  \\
  &  &($6.694\times 10^{-6}$)&  \\
after\_treated\_1st $\times $ maturity $\times $ moneyness\_less\_1&  &$-2.72\times 10^{-5}$$^{***}$&  \\
  &  &($9.362\times 10^{-6}$)&  \\
after\_treated\_last&  &  &-0.0038\\
  &  &  &(0.0028)\\
after\_treated\_last $\times $ moneyness\_more\_1&  &  &0.0044$^{*}$\\
  &  &  &(0.0024)\\
after\_treated\_last $\times $ maturity&  &  &$4.16\times 10^{-6}$\\
  &  &  &($6.036\times 10^{-6}$)\\
after\_treated\_last $\times $ moneyness\_less\_1&  &  &0.0043\\
  &  &  &(0.0030)\\
after\_treated\_last $\times $ moneyness\_more\_1 $\times $ maturity&  &  &$-7.041\times 10^{-6}$\\
  &  &  &($5.417\times 10^{-6}$)\\
after\_treated\_last $\times $ maturity $\times $ moneyness\_less\_1&  &  &$-6.604\times 10^{-6}$\\
  &  &  &($7.013\times 10^{-6}$)\\

\hline
\emph{Fixed-effects}&  & & \\

ticker&Yes&Yes&Yes\\
date&Yes&Yes&Yes\\
call&Yes&Yes&Yes\\

\hline
\emph{Fit statistics}&  & & \\
Observations& 6,095,802&6,095,802&6,095,802\\
R$^2$ & 0.05067&0.05076&0.0506\\
Within R$^2$ & 0.008&0.0081&0.00793\\

\hline\hline
\multicolumn{4}{l}{\emph{One-way (ticker) standard-errors in parentheses}}\\
\multicolumn{4}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\

\end{tabular}



==> tables/table_rn_kurtosis_results.tex <==
\begin{tabular}{lcccccc}
\tabularnewline\hline\hline

Dependent Variable:&\multicolumn{6}{c}{rn\_kurtosis}\\

Model:&(1)&(2)&(3)&(4)&(5)&(6)\\

\hline
\emph{Variables}&  & & & & & \\

treated&-86058.4$^{***}$&  &  &  &  &  \\
  &(6254.6)&  &  &  &  &  \\
treated $\times $ maturity\_cut(1,28]&  &-41666.7$^{***}$&  &  &  &  \\
  &  &(8031)&  &  &  &  \\
treated $\times $ maturity\_cut(28,60]&  &-89543.9$^{***}$&  &  &  &  \\
  &  &(6644.3)&  &  &  &  \\
treated $\times $ maturity\_cut(60,177]&  &-102243.9$^{***}$&  &  &  &  \\
  &  &(7269.3)&  &  &  &  \\
treated $\times $ maturity\_cut(177,950]&  &-114762.1$^{***}$&  &  &  &  \\
  &  &(7733.1)&  &  &  &  \\
after\_treated\_1st&  &  &-45122.2$^{***}$&  &  &  \\
  &  &  &(7018.5)&  &  &  \\
after\_treated\_1st $\times $ maturity\_cut(1,28]&  &  &  &14507.2&  &  \\
  &  &  &  &(10532.4)&  &  \\
after\_treated\_1st $\times $ maturity\_cut(28,60]&  &  &  &-32279.6$^{***}$&  &  \\
  &  &  &  &(8196.7)&  &  \\
after\_treated\_1st $\times $ maturity\_cut(60,177]&  &  &  &-72940.5$^{***}$&  &  \\
  &  &  &  &(7248.1)&  &  \\
after\_treated\_1st $\times $ maturity\_cut(177,950]&  &  &  &-89558.1$^{***}$&  &  \\
  &  &  &  &(7491.2)&  &  \\
after\_treated\_last&  &  &  &  &32336$^{***}$&  \\
  &  &  &  &  &(8087.9)&  \\
after\_treated\_last $\times $ maturity\_cut(1,28]&  &  &  &  &  &124278.1$^{***}$\\
  &  &  &  &  &  &(18768.1)\\
after\_treated\_last $\times $ maturity\_cut(28,60]&  &  &  &  &  &60495.3$^{***}$\\
  &  &  &  &  &  &(12068.1)\\
after\_treated\_last $\times $ maturity\_cut(60,177]&  &  &  &  &  &-16712.4$^{***}$\\
  &  &  &  &  &  &(6355.8)\\
after\_treated\_last $\times $ maturity\_cut(177,950]&  &  &  &  &  &-37563.4$^{***}$\\
  &  &  &  &  &  &(6759.6)\\

\hline
\emph{Fixed-effects}&  & & & & & \\

ticker&Yes&Yes&Yes&Yes&Yes&Yes\\
date&Yes&Yes&Yes&Yes&Yes&Yes\\

\hline
\emph{Fit statistics}&  & & & & & \\
Observations& 38,169&37,951&38,169&37,951&38,169&37,951\\
R$^2$ & 0.10872&0.11539&0.1011&0.11712&0.09984&0.11146\\
Within R$^2$ & 0.0109&0.01723&0.00244&0.01915&0.00105&0.01286\\

\hline\hline
\multicolumn{7}{l}{\emph{One-way (ticker) standard-errors in parentheses}}\\
\multicolumn{7}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\

\end{tabular}



==> tables/table_rn_mean_results.tex <==
\begin{tabular}{lcccccc}
\tabularnewline\hline\hline

Dependent Variable:&\multicolumn{6}{c}{rn\_mean}\\

Model:&(1)&(2)&(3)&(4)&(5)&(6)\\

\hline
\emph{Variables}&  & & & & & \\

treated&0.0573$^{***}$&  &  &  &  &  \\
  &(0.0087)&  &  &  &  &  \\
treated $\times $ maturity\_cut(1,28]&  &0.0031&  &  &  &  \\
  &  &(0.0091)&  &  &  &  \\
treated $\times $ maturity\_cut(28,60]&  &0.0297$^{***}$&  &  &  &  \\
  &  &(0.0087)&  &  &  &  \\
treated $\times $ maturity\_cut(60,177]&  &0.0807$^{***}$&  &  &  &  \\
  &  &(0.0112)&  &  &  &  \\
treated $\times $ maturity\_cut(177,950]&  &0.1295$^{***}$&  &  &  &  \\
  &  &(0.0142)&  &  &  &  \\
after\_treated\_1st&  &  &0.0315$^{***}$&  &  &  \\
  &  &  &(0.0073)&  &  &  \\
after\_treated\_1st $\times $ maturity\_cut(1,28]&  &  &  &-0.0155$^{*}$&  &  \\
  &  &  &  &(0.0081)&  &  \\
after\_treated\_1st $\times $ maturity\_cut(28,60]&  &  &  &0.0098&  &  \\
  &  &  &  &(0.0075)&  &  \\
after\_treated\_1st $\times $ maturity\_cut(60,177]&  &  &  &0.0507$^{***}$&  &  \\
  &  &  &  &(0.0095)&  &  \\
after\_treated\_1st $\times $ maturity\_cut(177,950]&  &  &  &0.0858$^{***}$&  &  \\
  &  &  &  &(0.0108)&  &  \\
after\_treated\_last&  &  &  &  &-0.0204$^{***}$&  \\
  &  &  &  &  &(0.0061)&  \\
after\_treated\_last $\times $ maturity\_cut(1,28]&  &  &  &  &  &-0.0565$^{***}$\\
  &  &  &  &  &  &(0.0080)\\
after\_treated\_last $\times $ maturity\_cut(28,60]&  &  &  &  &  &-0.0307$^{***}$\\
  &  &  &  &  &  &(0.0077)\\
after\_treated\_last $\times $ maturity\_cut(60,177]&  &  &  &  &  &-0.0060\\
  &  &  &  &  &  &(0.0093)\\
after\_treated\_last $\times $ maturity\_cut(177,950]&  &  &  &  &  &0.0115\\
  &  &  &  &  &  &(0.0094)\\

\hline
\emph{Fixed-effects}&  & & & & & \\

ticker&Yes&Yes&Yes&Yes&Yes&Yes\\
date&Yes&Yes&Yes&Yes&Yes&Yes\\

\hline
\emph{Fit statistics}&  & & & & & \\
Observations& 38,169&37,951&38,169&37,951&38,169&37,951\\
R$^2$ & 0.13381&0.14959&0.13066&0.14427&0.12999&0.13229\\
Within R$^2$ & 0.0048&0.02213&0.00119&0.01602&0.00042&0.00224\\

\hline\hline
\multicolumn{7}{l}{\emph{One-way (ticker) standard-errors in parentheses}}\\
\multicolumn{7}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\

\end{tabular}



==> tables/table_rn_sd_results.tex <==
\begin{tabular}{lcccccc}
\tabularnewline\hline\hline

Dependent Variable:&\multicolumn{6}{c}{rn\_sd}\\

Model:&(1)&(2)&(3)&(4)&(5)&(6)\\

\hline
\emph{Variables}&  & & & & & \\

treated&0.0723$^{***}$&  &  &  &  &  \\
  &(0.0031)&  &  &  &  &  \\
treated $\times $ maturity\_cut(1,28]&  &0.0391$^{***}$&  &  &  &  \\
  &  &(0.0041)&  &  &  &  \\
treated $\times $ maturity\_cut(28,60]&  &0.0545$^{***}$&  &  &  &  \\
  &  &(0.0036)&  &  &  &  \\
treated $\times $ maturity\_cut(60,177]&  &0.0949$^{***}$&  &  &  &  \\
  &  &(0.0038)&  &  &  &  \\
treated $\times $ maturity\_cut(177,950]&  &0.1100$^{***}$&  &  &  &  \\
  &  &(0.0043)&  &  &  &  \\
after\_treated\_1st&  &  &0.0428$^{***}$&  &  &  \\
  &  &  &(0.0032)&  &  &  \\
after\_treated\_1st $\times $ maturity\_cut(1,28]&  &  &  &0.0127$^{***}$&  &  \\
  &  &  &  &(0.0040)&  &  \\
after\_treated\_1st $\times $ maturity\_cut(28,60]&  &  &  &0.0256$^{***}$&  &  \\
  &  &  &  &(0.0037)&  &  \\
after\_treated\_1st $\times $ maturity\_cut(60,177]&  &  &  &0.0615$^{***}$&  &  \\
  &  &  &  &(0.0037)&  &  \\
after\_treated\_1st $\times $ maturity\_cut(177,950]&  &  &  &0.0742$^{***}$&  &  \\
  &  &  &  &(0.0038)&  &  \\
after\_treated\_last&  &  &  &  &-0.0243$^{***}$&  \\
  &  &  &  &  &(0.0022)&  \\
after\_treated\_last $\times $ maturity\_cut(1,28]&  &  &  &  &  &-0.0477$^{***}$\\
  &  &  &  &  &  &(0.0026)\\
after\_treated\_last $\times $ maturity\_cut(28,60]&  &  &  &  &  &-0.0400$^{***}$\\
  &  &  &  &  &  &(0.0026)\\
after\_treated\_last $\times $ maturity\_cut(60,177]&  &  &  &  &  &-0.0109$^{***}$\\
  &  &  &  &  &  &(0.0029)\\
after\_treated\_last $\times $ maturity\_cut(177,950]&  &  &  &  &  &0.0016\\
  &  &  &  &  &  &(0.0033)\\

\hline
\emph{Fixed-effects}&  & & & & & \\

ticker&Yes&Yes&Yes&Yes&Yes&Yes\\
date&Yes&Yes&Yes&Yes&Yes&Yes\\

\hline
\emph{Fit statistics}&  & & & & & \\
Observations& 38,169&37,951&38,169&37,951&38,169&37,951\\
R$^2$ & 0.36096&0.41747&0.31318&0.36989&0.29924&0.31075\\
Within R$^2$ & 0.09476&0.17312&0.02708&0.10559&0.00732&0.02163\\

\hline\hline
\multicolumn{7}{l}{\emph{One-way (ticker) standard-errors in parentheses}}\\
\multicolumn{7}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\

\end{tabular}



==> tables/table_rn_skewness_results.tex <==
\begin{tabular}{lcccccc}
\tabularnewline\hline\hline

Dependent Variable:&\multicolumn{6}{c}{rn\_skewness}\\

Model:&(1)&(2)&(3)&(4)&(5)&(6)\\

\hline
\emph{Variables}&  & & & & & \\

treated&-0.1635$^{***}$&  &  &  &  &  \\
  &(0.0325)&  &  &  &  &  \\
treated $\times $ maturity\_cut(1,28]&  &-0.0095&  &  &  &  \\
  &  &(0.0401)&  &  &  &  \\
treated $\times $ maturity\_cut(28,60]&  &0.0172&  &  &  &  \\
  &  &(0.0323)&  &  &  &  \\
treated $\times $ maturity\_cut(60,177]&  &-0.2604$^{***}$&  &  &  &  \\
  &  &(0.0455)&  &  &  &  \\
treated $\times $ maturity\_cut(177,950]&  &-0.4559$^{***}$&  &  &  &  \\
  &  &(0.0570)&  &  &  &  \\
after\_treated\_1st&  &  &-0.1209$^{***}$&  &  &  \\
  &  &  &(0.0312)&  &  &  \\
after\_treated\_1st $\times $ maturity\_cut(1,28]&  &  &  &-0.0023&  &  \\
  &  &  &  &(0.0381)&  &  \\
after\_treated\_1st $\times $ maturity\_cut(28,60]&  &  &  &0.0365&  &  \\
  &  &  &  &(0.0338)&  &  \\
after\_treated\_1st $\times $ maturity\_cut(60,177]&  &  &  &-0.2137$^{***}$&  &  \\
  &  &  &  &(0.0400)&  &  \\
after\_treated\_1st $\times $ maturity\_cut(177,950]&  &  &  &-0.3199$^{***}$&  &  \\
  &  &  &  &(0.0449)&  &  \\
after\_treated\_last&  &  &  &  &0.0421&  \\
  &  &  &  &  &(0.0271)&  \\
after\_treated\_last $\times $ maturity\_cut(1,28]&  &  &  &  &  &0.1119$^{**}$\\
  &  &  &  &  &  &(0.0437)\\
after\_treated\_last $\times $ maturity\_cut(28,60]&  &  &  &  &  &0.1459$^{***}$\\
  &  &  &  &  &  &(0.0360)\\
after\_treated\_last $\times $ maturity\_cut(60,177]&  &  &  &  &  &-0.0694$^{**}$\\
  &  &  &  &  &  &(0.0321)\\
after\_treated\_last $\times $ maturity\_cut(177,950]&  &  &  &  &  &-0.0230\\
  &  &  &  &  &  &(0.0332)\\

\hline
\emph{Fixed-effects}&  & & & & & \\

ticker&Yes&Yes&Yes&Yes&Yes&Yes\\
date&Yes&Yes&Yes&Yes&Yes&Yes\\

\hline
\emph{Fit statistics}&  & & & & & \\
Observations& 38,169&37,951&38,169&37,951&38,169&37,951\\
R$^2$ & 0.21418&0.23109&0.21296&0.22652&0.21208&0.21465\\
Within R$^2$ & 0.00279&0.02265&0.00124&0.01685&0.00013&0.00176\\

\hline\hline
\multicolumn{7}{l}{\emph{One-way (ticker) standard-errors in parentheses}}\\
\multicolumn{7}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\

\end{tabular}



==> tables/table_rnd_moments_after_treated_1st_linear_results.tex <==
\begin{tabular}{lcccc}
\tabularnewline\hline\hline

Dependent Variables:&rn\_mean&rn\_sd&rn\_skewness&rn\_kurtosis\\

Model:&(1)&(2)&(3)&(4)\\

\hline
\emph{Variables}&  & & & \\

after\_treated\_1st&-0.0004&-0.0022&0.0038&425.5\\
  &(0.0040)&(0.0025)&(0.0104)&(1065.5)\\
maturity\_minus\_78&0.0162$^{***}$&0.0723$^{***}$&0.0158$^{***}$&-12641.2$^{***}$\\
  &(0.0024)&(0.0016)&(0.0049)&(752.4)\\
after\_treated\_1st $\times $ maturity\_minus\_78&-0.0011&0.0051$^{**}$&0.0218$^{***}$&-2379$^{***}$\\
  &(0.0032)&(0.0022)&(0.0067)&(903.7)\\

\hline
\emph{Fixed-effects}&  & & & \\

ticker&Yes&Yes&Yes&Yes\\
date&Yes&Yes&Yes&Yes\\
call&Yes&Yes&Yes&Yes\\

\hline
\emph{Fit statistics}&  & & & \\
Observations& 50,350&50,350&50,350&50,350\\
R$^2$ & 0.26876&0.59048&0.15267&0.2975\\
Within R$^2$ & 0.00871&0.41291&0.00668&0.12768\\

\hline\hline
\multicolumn{5}{l}{\emph{One-way (ticker) standard-errors in parentheses}}\\
\multicolumn{5}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\

\end{tabular}



==> tables/table_rnd_moments_after_treated_1st_results.tex <==
\begin{tabular}{lcccc}
\tabularnewline\hline\hline

Dependent Variables:&rn\_mean&rn\_sd&rn\_skewness&rn\_kurtosis\\

Model:&(1)&(2)&(3)&(4)\\

\hline
\emph{Variables}&  & & & \\

maturity\_cut(29,71]&-0.0246$^{***}$&0.0215$^{***}$&0.0443$^{***}$&-8216.6$^{***}$\\
  &(0.0025)&(0.0014)&(0.0077)&(858.9)\\
maturity\_cut(71,189]&0.0120$^{***}$&0.0911$^{***}$&-0.0070&-22546.4$^{***}$\\
  &(0.0033)&(0.0023)&(0.0080)&(1360.2)\\
maturity\_cut(189,946]&0.0200$^{***}$&0.1327$^{***}$&0.0199$^{**}$&-27202.6$^{***}$\\
  &(0.0038)&(0.0029)&(0.0086)&(1665.9)\\
after\_treated\_1st $\times $ maturity\_cut(1,29]&-0.0059&-0.0022&-0.0288$^{**}$&1867.8\\
  &(0.0045)&(0.0030)&(0.0138)&(1849.6)\\
after\_treated\_1st $\times $ maturity\_cut(29,71]&0.0025&-0.0106$^{***}$&0.0179&3981$^{***}$\\
  &(0.0050)&(0.0030)&(0.0127)&(1389.4)\\
after\_treated\_1st $\times $ maturity\_cut(71,189]&0.0063&0.0021&0.0226$^{**}$&-3219.5$^{***}$\\
  &(0.0049)&(0.0026)&(0.0105)&(902.6)\\
after\_treated\_1st $\times $ maturity\_cut(189,946]&-0.0040&0.0060$^{*}$&0.0251$^{**}$&-2876.6$^{***}$\\
  &(0.0049)&(0.0031)&(0.0113)&(1015.5)\\

\hline
\emph{Fixed-effects}&  & & & \\

ticker&Yes&Yes&Yes&Yes\\
date&Yes&Yes&Yes&Yes\\
call&Yes&Yes&Yes&Yes\\

\hline
\emph{Fit statistics}&  & & & \\
Observations& 49,994&49,994&49,994&49,994\\
R$^2$ & 0.27869&0.64465&0.15796&0.37039\\
Within R$^2$ & 0.02179&0.48965&0.0128&0.21872\\

\hline\hline
\multicolumn{5}{l}{\emph{One-way (ticker) standard-errors in parentheses}}\\
\multicolumn{5}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\

\end{tabular}



==> tables/table_rnd_moments_after_treated_last_linear_results.tex <==
\begin{tabular}{lcccc}
\tabularnewline\hline\hline

Dependent Variables:&rn\_mean&rn\_sd&rn\_skewness&rn\_kurtosis\\

Model:&(1)&(2)&(3)&(4)\\

\hline
\emph{Variables}&  & & & \\

after\_treated\_last&-0.0015&-0.0002&-0.0018&-1113.3\\
  &(0.0029)&(0.0018)&(0.0075)&(798.3)\\
maturity\_minus\_78&0.0151$^{***}$&0.0754$^{***}$&0.0315$^{***}$&-14238.1$^{***}$\\
  &(0.0019)&(0.0015)&(0.0048)&(910.5)\\
after\_treated\_last $\times $ maturity\_minus\_78&0.0017&0.0031$^{*}$&-0.0042&-296.8\\
  &(0.0025)&(0.0019)&(0.0055)&(693.2)\\

\hline
\emph{Fixed-effects}&  & & & \\

ticker&Yes&Yes&Yes&Yes\\
date&Yes&Yes&Yes&Yes\\
call&Yes&Yes&Yes&Yes\\

\hline
\emph{Fit statistics}&  & & & \\
Observations& 50,350&50,350&50,350&50,350\\
R$^2$ & 0.26876&0.59025&0.15206&0.29695\\
Within R$^2$ & 0.00872&0.41258&0.00597&0.12699\\

\hline\hline
\multicolumn{5}{l}{\emph{One-way (ticker) standard-errors in parentheses}}\\
\multicolumn{5}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\

\end{tabular}



==> tables/table_rnd_moments_after_treated_last_results.tex <==
\begin{tabular}{lcccc}
\tabularnewline\hline\hline

Dependent Variables:&rn\_mean&rn\_sd&rn\_skewness&rn\_kurtosis\\

Model:&(1)&(2)&(3)&(4)\\

\hline
\emph{Variables}&  & & & \\

maturity\_cut(29,71]&-0.0193$^{***}$&0.0164$^{***}$&0.0765$^{***}$&-6918.1$^{***}$\\
  &(0.0023)&(0.0012)&(0.0069)&(971.9)\\
maturity\_cut(71,189]&0.0205$^{***}$&0.0934$^{***}$&0.0278$^{***}$&-25631.5$^{***}$\\
  &(0.0032)&(0.0021)&(0.0069)&(1684.5)\\
maturity\_cut(189,946]&0.0211$^{***}$&0.1372$^{***}$&0.0576$^{***}$&-30207.1$^{***}$\\
  &(0.0034)&(0.0030)&(0.0088)&(2021.2)\\
after\_treated\_last $\times $ maturity\_cut(1,29]&-0.0022&-0.0021&-0.0006&-190\\
  &(0.0034)&(0.0020)&(0.0103)&(1424.8)\\
after\_treated\_last $\times $ maturity\_cut(29,71]&0.0005&-0.0048$^{**}$&-0.0005&100.1\\
  &(0.0038)&(0.0024)&(0.0096)&(1088.6)\\
after\_treated\_last $\times $ maturity\_cut(71,189]&-0.0056&0.0009&-0.0008&-1892.6$^{***}$\\
  &(0.0039)&(0.0022)&(0.0088)&(664.7)\\
after\_treated\_last $\times $ maturity\_cut(189,946]&0.0006&0.0048$^{*}$&-0.0046&-1722.1$^{**}$\\
  &(0.0041)&(0.0025)&(0.0088)&(723.6)\\

\hline
\emph{Fixed-effects}&  & & & \\

ticker&Yes&Yes&Yes&Yes\\
date&Yes&Yes&Yes&Yes\\
call&Yes&Yes&Yes&Yes\\

\hline
\emph{Fit statistics}&  & & & \\
Observations& 49,994&49,994&49,994&49,994\\
R$^2$ & 0.27843&0.64389&0.1567&0.36815\\
Within R$^2$ & 0.02143&0.48856&0.01132&0.21595\\

\hline\hline
\multicolumn{5}{l}{\emph{One-way (ticker) standard-errors in parentheses}}\\
\multicolumn{5}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\

\end{tabular}



==> tables/table_rnd_moments_treated_linear_results.tex <==
\begin{tabular}{lcccc}
\tabularnewline\hline\hline

Dependent Variables:&rn\_mean&rn\_sd&rn\_skewness&rn\_kurtosis\\

Model:&(1)&(2)&(3)&(4)\\

\hline
\emph{Variables}&  & & & \\

treated&0.0043&-0.0009&0.0047&1003.3\\
  &(0.0032)&(0.0019)&(0.0087)&(885.6)\\
maturity\_minus\_78&0.0155$^{***}$&0.0736$^{***}$&0.0178$^{***}$&-12993.7$^{***}$\\
  &(0.0021)&(0.0014)&(0.0043)&(697.2)\\
treated $\times $ maturity\_minus\_78&-0.0002&0.0039$^{*}$&0.0226$^{***}$&-2229$^{***}$\\
  &(0.0030)&(0.0021)&(0.0059)&(825)\\

\hline
\emph{Fixed-effects}&  & & & \\

ticker&Yes&Yes&Yes&Yes\\
date&Yes&Yes&Yes&Yes\\
call&Yes&Yes&Yes&Yes\\

\hline
\emph{Fit statistics}&  & & & \\
Observations& 50,350&50,350&50,350&50,350\\
R$^2$ & 0.26883&0.59038&0.15283&0.29752\\
Within R$^2$ & 0.00881&0.41276&0.00687&0.1277\\

\hline\hline
\multicolumn{5}{l}{\emph{One-way (ticker) standard-errors in parentheses}}\\
\multicolumn{5}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\

\end{tabular}



==> tables/table_rnd_moments_treated_results.tex <==
\begin{tabular}{lcccc}
\tabularnewline\hline\hline

Dependent Variables:&rn\_mean&rn\_sd&rn\_skewness&rn\_kurtosis\\

Model:&(1)&(2)&(3)&(4)\\

\hline
\emph{Variables}&  & & & \\

maturity\_cut(29,71]&-0.0233$^{***}$&0.0202$^{***}$&0.0430$^{***}$&-8218.4$^{***}$\\
  &(0.0022)&(0.0012)&(0.0066)&(822.5)\\
maturity\_cut(71,189]&0.0128$^{***}$&0.0926$^{***}$&-0.0061&-23522.6$^{***}$\\
  &(0.0030)&(0.0020)&(0.0068)&(1283.2)\\
maturity\_cut(189,946]&0.0204$^{***}$&0.1356$^{***}$&0.0226$^{***}$&-28180.8$^{***}$\\
  &(0.0035)&(0.0027)&(0.0075)&(1544)\\
treated $\times $ maturity\_cut(1,29]&-0.0007&-0.0001&-0.0348$^{***}$&1965.2\\
  &(0.0038)&(0.0024)&(0.0123)&(1566.2)\\
treated $\times $ maturity\_cut(29,71]&0.0069$^{*}$&-0.0076$^{***}$&0.0228$^{**}$&4392.6$^{***}$\\
  &(0.0041)&(0.0025)&(0.0111)&(1304.9)\\
treated $\times $ maturity\_cut(71,189]&0.0125$^{***}$&0.0023&0.0246$^{***}$&-2348$^{***}$\\
  &(0.0046)&(0.0021)&(0.0095)&(669.1)\\
treated $\times $ maturity\_cut(189,946]&0.0009&0.0045$^{*}$&0.0243$^{***}$&-1978.6$^{**}$\\
  &(0.0045)&(0.0025)&(0.0093)&(834.7)\\

\hline
\emph{Fixed-effects}&  & & & \\

ticker&Yes&Yes&Yes&Yes\\
date&Yes&Yes&Yes&Yes\\
call&Yes&Yes&Yes&Yes\\

\hline
\emph{Fit statistics}&  & & & \\
Observations& 49,994&49,994&49,994&49,994\\
R$^2$ & 0.27888&0.64427&0.1586&0.37021\\
Within R$^2$ & 0.02205&0.48911&0.01355&0.21849\\

\hline\hline
\multicolumn{5}{l}{\emph{One-way (ticker) standard-errors in parentheses}}\\
\multicolumn{5}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\

\end{tabular}



==> tables/table_treatment_after_treated_1st_results.tex <==
\begin{tabular}{lcccccccc}
\tabularnewline\hline\hline

Dependent Variables:&\multicolumn{2}{c}{rn\_mean}&\multicolumn{2}{c}{rn\_sd}&\multicolumn{2}{c}{rn\_skewness}&\multicolumn{2}{c}{rn\_kurtosis}\\

Model:&(1)&(2)&(3)&(4)&(5)&(6)&(7)&(8)\\

\hline
\emph{Variables}&  & & & & & & & \\

after\_treated\_1st&0.0315$^{***}$&  &0.0428$^{***}$&  &-0.1209$^{***}$&  &-45122.2$^{***}$&  \\
  &(0.0073)&  &(0.0032)&  &(0.0312)&  &(7018.5)&  \\
after\_treated\_1st $\times $ maturity\_cut(1,28]&  &-0.0155$^{*}$&  &0.0127$^{***}$&  &-0.0023&  &14507.2\\
  &  &(0.0081)&  &(0.0040)&  &(0.0381)&  &(10532.4)\\
after\_treated\_1st $\times $ maturity\_cut(28,60]&  &0.0098&  &0.0256$^{***}$&  &0.0365&  &-32279.6$^{***}$\\
  &  &(0.0075)&  &(0.0037)&  &(0.0338)&  &(8196.7)\\
after\_treated\_1st $\times $ maturity\_cut(60,177]&  &0.0507$^{***}$&  &0.0615$^{***}$&  &-0.2137$^{***}$&  &-72940.5$^{***}$\\
  &  &(0.0095)&  &(0.0037)&  &(0.0400)&  &(7248.1)\\
after\_treated\_1st $\times $ maturity\_cut(177,950]&  &0.0858$^{***}$&  &0.0742$^{***}$&  &-0.3199$^{***}$&  &-89558.1$^{***}$\\
  &  &(0.0108)&  &(0.0038)&  &(0.0449)&  &(7491.2)\\

\hline
\emph{Fixed-effects}&  & & & & & & & \\

ticker&Yes&Yes&Yes&Yes&Yes&Yes&Yes&Yes\\
date&Yes&Yes&Yes&Yes&Yes&Yes&Yes&Yes\\

\hline
\emph{Fit statistics}&  & & & & & & & \\
Observations& 38,169&37,951&38,169&37,951&38,169&37,951&38,169&37,951\\
R$^2$ & 0.13066&0.14427&0.31318&0.36989&0.21296&0.22652&0.1011&0.11712\\
Within R$^2$ & 0.00119&0.01602&0.02708&0.10559&0.00124&0.01685&0.00244&0.01915\\

\hline\hline
\multicolumn{9}{l}{\emph{One-way (ticker) standard-errors in parentheses}}\\
\multicolumn{9}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\

\end{tabular}



==> tables/table_treatment_after_treated_last_results.tex <==
\begin{tabular}{lcccccccc}
\tabularnewline\hline\hline

Dependent Variables:&\multicolumn{2}{c}{rn\_mean}&\multicolumn{2}{c}{rn\_sd}&\multicolumn{2}{c}{rn\_skewness}&\multicolumn{2}{c}{rn\_kurtosis}\\

Model:&(1)&(2)&(3)&(4)&(5)&(6)&(7)&(8)\\

\hline
\emph{Variables}&  & & & & & & & \\

after\_treated\_last&-0.0204$^{***}$&  &-0.0243$^{***}$&  &0.0421&  &32336$^{***}$&  \\
  &(0.0061)&  &(0.0022)&  &(0.0271)&  &(8087.9)&  \\
after\_treated\_last $\times $ maturity\_cut(1,28]&  &-0.0565$^{***}$&  &-0.0477$^{***}$&  &0.1119$^{**}$&  &124278.1$^{***}$\\
  &  &(0.0080)&  &(0.0026)&  &(0.0437)&  &(18768.1)\\
after\_treated\_last $\times $ maturity\_cut(28,60]&  &-0.0307$^{***}$&  &-0.0400$^{***}$&  &0.1459$^{***}$&  &60495.3$^{***}$\\
  &  &(0.0077)&  &(0.0026)&  &(0.0360)&  &(12068.1)\\
after\_treated\_last $\times $ maturity\_cut(60,177]&  &-0.0060&  &-0.0109$^{***}$&  &-0.0694$^{**}$&  &-16712.4$^{***}$\\
  &  &(0.0093)&  &(0.0029)&  &(0.0321)&  &(6355.8)\\
after\_treated\_last $\times $ maturity\_cut(177,950]&  &0.0115&  &0.0016&  &-0.0230&  &-37563.4$^{***}$\\
  &  &(0.0094)&  &(0.0033)&  &(0.0332)&  &(6759.6)\\

\hline
\emph{Fixed-effects}&  & & & & & & & \\

ticker&Yes&Yes&Yes&Yes&Yes&Yes&Yes&Yes\\
date&Yes&Yes&Yes&Yes&Yes&Yes&Yes&Yes\\

\hline
\emph{Fit statistics}&  & & & & & & & \\
Observations& 38,169&37,951&38,169&37,951&38,169&37,951&38,169&37,951\\
R$^2$ & 0.12999&0.13229&0.29924&0.31075&0.21208&0.21465&0.09984&0.11146\\
Within R$^2$ & 0.00042&0.00224&0.00732&0.02163&0.00013&0.00176&0.00105&0.01286\\

\hline\hline
\multicolumn{9}{l}{\emph{One-way (ticker) standard-errors in parentheses}}\\
\multicolumn{9}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\

\end{tabular}



==> tables/table_treatment_treated_results.tex <==
\begin{tabular}{lcccccccc}
\tabularnewline\hline\hline

Dependent Variables:&\multicolumn{2}{c}{rn\_mean}&\multicolumn{2}{c}{rn\_sd}&\multicolumn{2}{c}{rn\_skewness}&\multicolumn{2}{c}{rn\_kurtosis}\\

Model:&(1)&(2)&(3)&(4)&(5)&(6)&(7)&(8)\\

\hline
\emph{Variables}&  & & & & & & & \\

treated&0.0573$^{***}$&  &0.0723$^{***}$&  &-0.1635$^{***}$&  &-86058.4$^{***}$&  \\
  &(0.0087)&  &(0.0031)&  &(0.0325)&  &(6254.6)&  \\
treated $\times $ maturity\_cut(1,28]&  &0.0031&  &0.0391$^{***}$&  &-0.0095&  &-41666.7$^{***}$\\
  &  &(0.0091)&  &(0.0041)&  &(0.0401)&  &(8031)\\
treated $\times $ maturity\_cut(28,60]&  &0.0297$^{***}$&  &0.0545$^{***}$&  &0.0172&  &-89543.9$^{***}$\\
  &  &(0.0087)&  &(0.0036)&  &(0.0323)&  &(6644.3)\\
treated $\times $ maturity\_cut(60,177]&  &0.0807$^{***}$&  &0.0949$^{***}$&  &-0.2604$^{***}$&  &-102243.9$^{***}$\\
  &  &(0.0112)&  &(0.0038)&  &(0.0455)&  &(7269.3)\\
treated $\times $ maturity\_cut(177,950]&  &0.1295$^{***}$&  &0.1100$^{***}$&  &-0.4559$^{***}$&  &-114762.1$^{***}$\\
  &  &(0.0142)&  &(0.0043)&  &(0.0570)&  &(7733.1)\\

\hline
\emph{Fixed-effects}&  & & & & & & & \\

ticker&Yes&Yes&Yes&Yes&Yes&Yes&Yes&Yes\\
date&Yes&Yes&Yes&Yes&Yes&Yes&Yes&Yes\\

\hline
\emph{Fit statistics}&  & & & & & & & \\
Observations& 38,169&37,951&38,169&37,951&38,169&37,951&38,169&37,951\\
R$^2$ & 0.13381&0.14959&0.36096&0.41747&0.21418&0.23109&0.10872&0.11539\\
Within R$^2$ & 0.0048&0.02213&0.09476&0.17312&0.00279&0.02265&0.0109&0.01723\\

\hline\hline
\multicolumn{9}{l}{\emph{One-way (ticker) standard-errors in parentheses}}\\
\multicolumn{9}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\

\end{tabular}



==> tables/trading_tails.tex <==
\begin{tabular}{lcccc}
\toprule
                         & \multicolumn{1}{c}{$K/S<0.5$} & \multicolumn{1}{c}{$K/S<0.2$} & \multicolumn{1}{c}{strike\_over\_price\_more\_1\_5} & \multicolumn{1}{c}{strike\_over\_price\_more\_1\_8} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5}
                         &                                                 (1) &                                                 (2) &                                                 (3) &  
                                               (4) \\
\midrule
maturity\_100            &                                            0.004*** &                                            0.001*** &                                            0.003*** &  
                                          0.001*** \\
                         &                                             (0.000) &                                             (0.000) &                                             (0.000) &  
                                           (0.000) \\
treated                  &                                             0.009** &                                               0.001 &                                               0.001 &  
                                             0.004 \\
                         &                                             (0.003) &                                             (0.001) &                                             (0.005) &  
                                           (0.003) \\
treated \& maturity\_100 &                                            -0.001** &                                              -0.000 &                                              -0.000 &  
                                          -0.001** \\
                         &                                             (0.000) &                                             (0.000) &                                             (0.000) &  
                                           (0.000) \\
\midrule
date                     &                                                 Yes &                                                 Yes &                                                 Yes &  
                                               Yes \\
ticker                   &                                                 Yes &                                                 Yes &                                                 Yes &  
                                               Yes \\
\midrule
Estimator                &                                                 OLS &                                                 OLS &                                                 OLS &  
                                               OLS \\
\midrule
$N$                      &                                          16,842,463 &                                          16,842,463 &                                          16,839,339 &  
                                        16,839,339 \\
$R^2$                    &                                               0.054 &                                               0.035 &                                               0.116 &  
                                             0.091 \\
\bottomrule
\end{tabular}
